Nonequilibrium path-ensemble averages for symmetric protocols

According to the nonequilibrium work relations, path-ensembles generated by irreversible processes in which a system is driven out of equilibrium according to a predetermined protocol may be used to compute equilibrium free energy differences and expectation values. Estimation has previously been improved by considering data collected from the reverse process, which starts in equilibrium in the final thermodynamic state of the forward process and is driven according to the time-reversed protocol. Here, we develop a theoretically rigorous statistical estimator for nonequilibrium path-ensemble averages specialized for symmetric protocols, in which forward and reverse processes are identical. The estimator is tested with a number of model systems: a symmetric 1D potential, an asymmetric 1D potential, the unfolding of deca-alanine, separating a host-guest system, and translocating a potassium ion through a gramicidin A ion channel. When reconstructing free energies using data from symmetric protocols, the new estimator outperforms existing rigorous unidirectional and bidirectional estimators, converging more quickly and resulting in smaller error. However, in most cases, using the bidirectional estimator with data from a forward and reverse pair of asymmetric protocols outperforms the corresponding symmetric protocol and estimator with the same amount of simulation time. Hence, the new estimator is only recommended when the bidirectional estimator is not feasible or is expected to perform poorly. The symmetric estimator has similar performance to a unidirectional protocol of half the length and twice the number of trajectories.

==> optimization.tex <==
The path-ensemble average of a functional $\mathcal{F}[\Gamma]$ that depends on a path $\Gamma$ is defined as,
%
\begin{eqnarray}
\label{path_ensemble_av}
\E{\mathcal{F}} = \frac{\int \mathcal{F}[\Gamma] \rho_F[\Gamma] d\Gamma}
{\int \rho_F[\Gamma] d\Gamma} ,
\end{eqnarray}
%
where $\rho_F[\Gamma]$ is the probability density of the path in the forward process.
For simplicity $\rho_F[\Gamma]$ incorporates 
both the probability of the phase space point in the initial state 
and of the propagation through time for the duration of the process.
Integrals are over all possible paths.
Each integral in Equation \ref{path_ensemble_av} can be expressed as a linear combination,
\begin{eqnarray}
\label{eq:path_ensemble_linear_combination}
\E{\mathcal{F}} = 
\frac{\int \alpha[\Gamma] \mathcal{F}[\Gamma] \rho_F[\Gamma] d\Gamma + 
\int (1 - \alpha[\Gamma]) \mathcal{F}[\Gamma] \rho_F[\Gamma] d\Gamma}
{\int \alpha[\Gamma] \rho_F[\Gamma] d\Gamma +
\int (1 - \alpha[\Gamma]) \rho_F[\Gamma] d\Gamma},
\end{eqnarray}
where $\alpha[\Gamma]$ is a weighting factor. {\color{red} DELETE: We will select $\alpha[\Gamma]$ in a manner that minimizes the asymptotic variance of the path-ensemble average.}
{\color{blue} $\alpha[\Gamma]$ can be chosen to minimized the asymptotic variance of the path-ensemble average.}

For one of the integrals in each of sums, the integral over the path $\Gamma$ can be substituted for by an integral over the path $\tilde{\Gamma}$.
Assuming that the integrator is symplectic and because the initial and final states are the same, 
the Jacobian for the transformation is unity. The substitution leads to,
\begin{eqnarray}
\label{eq:path_ensemble_substitution}
\E{\mathcal{F}} = 
\frac{\int \alpha[\Gamma] \mathcal{F}[\Gamma] \rho_F[\Gamma] d\Gamma + 
\int (1 - \alpha[\tilde{\Gamma}]) \mathcal{F}[\tilde{\Gamma}] \rho_F[\tilde{\Gamma}] d\tilde{\Gamma}}
{\int \alpha[\Gamma] \rho_F[\Gamma] d\Gamma +
\int (1 - \alpha[\tilde{\Gamma}]) \rho_F[\tilde{\Gamma}] d\tilde{\Gamma}}.
\end{eqnarray}

% {\color{red} To get from Eq. \ref{eq:path_ensemble_linear_combination} to Eq. \ref{eq:path_ensemble_substitution}, do we make an assumption that (i) $\rho_F[\Gamma] d\Gamma = \rho_F[\tilde{\Gamma}] d\tilde{\Gamma}$ and that (ii) $(1 - \alpha[\Gamma]) \mathcal{F}[\Gamma] = (1 - \alpha[\tilde{\Gamma}]) \mathcal{F}[\tilde{\Gamma}]$? (i) is apparently true, but it is not so evident for me that (ii) is true.}

As a key step towards deriving his eponymous fluctuation theorem, Crooks \cite{Crooks1998,Crooks2000} showed that probability densities in forward and reverse path-ensembles are related by,
\begin{eqnarray}
\label{eq:path_rho_ratio}
\frac{\rho_F[\Gamma]}{\rho_R[\tilde{\Gamma}]} = e^{\beta \left( W - \Delta F \right)},
\end{eqnarray}
where $\beta = (k_B T)^{-1}$ is the inverse product of Boltzmann's constant $k_B$ and the temperature $T$, $W$ is the total work done on the system during the forward process, and $\Delta F$ % = F_{\tau} - F_0
is the change in free energy between the initial and final thermodynamic state of the forward process. For the symmetric protocols considered in this work, the free energy difference is zero, $\Delta F = 0$. Also, because forward and reverse processes are equivalent, $\rho_F[\Gamma] = \rho_R[\Gamma]$. Therefore, in the special case of symmetric protocols, Equation \ref{eq:path_rho_ratio} may be simplified into,
\begin{eqnarray}
\label{eq:path_rho_ratio_simplified}
\frac{\rho_F[\Gamma]}{\rho_F[\tilde{\Gamma}]} = e^{\beta W },
\end{eqnarray}
Substituting Equation \ref{eq:path_rho_ratio_simplified} into Equation \ref{eq:path_ensemble_substitution} leads to,
\begin{eqnarray}
\label{eq:path_ensemble_integral}
\E{\mathcal{F}} = 
\frac{\int \left[ \alpha[\Gamma] \mathcal{F}[\Gamma] + (1 - \alpha[\tilde{\Gamma}]) \mathcal{F}[\tilde{\Gamma}] e^{-\beta W} \right] \rho_F[\Gamma] d\Gamma}
{\int \left[ \alpha[\Gamma] + (1 - \alpha[\tilde{\Gamma}]) e^{-\beta W} \right] \rho_F[\Gamma] d\Gamma},
\end{eqnarray}
An estimator for the path-ensemble average, $\overline{\mathcal{F}}$, 
may be obtained by multiplying and dividing by $\int \rho_F[\Gamma] d\Gamma$ and using the sample mean for expectation values in both the numerator and denominator,
\begin{eqnarray}
\label{eq:path_ensemble_estimator_alpha}
\overline{\mathcal{F}} = 
\frac{\sum\limits_{n=1}^N \left[ \alpha[\Gamma_n] \mathcal{F}[\Gamma_n] + (1 - \alpha[\tilde{\Gamma}_n]) \mathcal{F}[\tilde{\Gamma}_n] e^{-\beta W[\Gamma_n]} \right] }
{\sum\limits_{n=1}^N \left[ \alpha[\Gamma_n] + (1 - \alpha[\tilde{\Gamma}_n]) e^{-\beta W[\Gamma_n]} \right] },
\end{eqnarray}
where $\Gamma_n$ is the $n^{th}$ of $N$ sampled trajectories.

{\color{blue} Minimizing the asymptotic variance of $\overline{\mathcal{F}}$ with respect to $\alpha[\Gamma]$ to select an optimal $\alpha[\Gamma]$ will be the subject of future work. Here, for simplicity, we choose $\alpha[\Gamma] = \frac{1}{2}$, and Equation \ref{eq:path_ensemble_estimator_alpha} becomes
\begin{eqnarray}
\label{eq:symmetric_estimator_alpha_12}
\overline{\mathcal{F}} = 
\frac{\sum\limits_{n=1}^N \left( \mathcal{F}[\Gamma_n] +  \mathcal{F}[\tilde{\Gamma}_n] e^{-\beta W[\Gamma_n]} \right) }
{\sum\limits_{n=1}^N \left( 1 + e^{-\beta W[\Gamma_n]} \right)}.
\end{eqnarray}
}

{\color{red} DELETE: Of the numerous possible choices for $\alpha[\Gamma]$, we would like to select a weighting functional that minimizes the error of estimated nonequilibrium path-ensemble averages.
In the limit of large sample sizes, the error should be Gaussian.
The asymptotic variance of Equation \ref{eq:path_ensemble_estimator_alpha} may be determined via error propagation based on a first-order Taylor series expansion. 
To simplify our expressions, let us define the functionals,
\begin{eqnarray}
A[\Gamma] &=& \alpha[\Gamma] \mathcal{F}[\Gamma] + (1 - \alpha[\tilde{\Gamma}]) \mathcal{F}[\tilde{\Gamma}] e^{-\beta W} \\
B[\Gamma] &=& \alpha[\Gamma] + (1 - \alpha[\tilde{\Gamma}]) e^{-\beta W}.
\end{eqnarray}
Sample mean estimators for the expectation values of A and B are
\begin{eqnarray}
\label{eq:A_and_B}
\overline{A} &=& \frac{1}{N} \sum_{n=0}^N A[\Gamma_n] \\
\overline{B} &=& \frac{1}{N} \sum_{n=0}^N B[\Gamma_n].
\end{eqnarray}
These estimators deviate from their true expectations, 
such that $\overline{A} = \E{A} - \Delta \overline{A}$ and $\overline{B} = \E{B} - \Delta \overline{B}$.
Equation \ref{eq:path_ensemble_estimator_alpha} may be written as a function of these deviations. A first-order Taylor series expansion leads to,
\begin{eqnarray}
\overline{\mathcal{F}} 
&=& \frac{\overline{A}}{\overline{B}} = \frac{\E{A} - \Delta \overline{A}}{\E{B} - \Delta \overline{B}} \nonumber \\
&\approx& \E{F} + \frac{1}{\E{B}} \Delta \overline{A} - \frac{\E{A}}{\E{B}^2} \Delta \overline{B}
\end{eqnarray}
Based on this approximation, the variance $\sigma^2[\overline{F}] \equiv \E{(\overline{F} - \E{F})^2}$ of Equation \ref{eq:path_ensemble_estimator_alpha} is,
\begin{eqnarray}
\label{eq:var_A_and_B}
\sigma^2[\overline{F}]
&=& \E{ \left( \frac{1}{\E{B}} \Delta \overline{A} - \frac{\E{A}}{\E{B}^2} \Delta \overline{B} \right)^2 } \nonumber \\
% &=& \E{ \frac{1}{\E{B}^2} \Delta \overline{A}^2 + \frac{\E{A}^2}{\E{B}^4} \Delta \overline{B}^2 - 2 \frac{\E{A}}{\E{B}^3} \Delta \overline{A} \Delta \overline{B} } \nonumber \\
&=& \frac{\E{\mathcal F}^2}{N} \left[ \frac{\sigma^2[A]}{\E{A}^2} + \frac{\sigma^2[B]}{\E{B}^2}  - 2 \frac{\sigma^2[A,B]}{\E{A} \E{B}} \right] \nonumber \\
&=& \frac{\E{\mathcal F}^2}{N} \left[ \frac{\E{A^2}}{\E{A}^2} + \frac{\E{B}^2}{\E{B}^2}  - 2 \frac{\E{AB}}{\E{A} \E{B}} \right]
\end{eqnarray}
Equations \ref{eq:A_and_B} to \ref{eq:var_A_and_B} are similar to a derivation in the supplementary material of a previous paper \cite{Minh2009b}.
}
